BT-Nets: Simplifying Deep Neural Networks via Block Term Decomposition

Recently, deep neural networks (DNNs) have been regarded as the state-of-the-art classification methods in a wide range of applications, especially in image classification. Despite the success, the huge number of parameters blocks its deployment to situations with light computing resources. Researchers resort to the redundancy in the weights of DNNs and attempt to find how fewer parameters can be chosen while preserving the accuracy at the same time. Although several promising results have been shown along this research line, most existing methods either fail to significantly compress a well-trained deep network or require a heavy fine-tuning process for the compressed network to regain the original performance. In this paper, we propose the \textit{Block Term} networks (BT-nets) in which the commonly used fully-connected layers (FC-layers) are replaced with block term layers (BT-layers). In BT-layers, the inputs and the outputs are reshaped into two low-dimensional high-order tensors, then block-term decomposition is applied as tensor operators to connect them. We conduct extensive experiments on benchmark datasets to demonstrate that BT-layers can achieve a very large compression ratio on the number of parameters while preserving the representation power of the original FC-layers as much as possible. Specifically, we can get a higher performance while requiring fewer parameters compared with the tensor train method.

==> related.tex <==
\section{Related Work}
% \begin{itemize}
%     \item  Deep learning literature
%     \item NN approximation: binary net, hash net, tt net, tensor switch net, 
%     \item Tensor networks variants: CP, TT, Tucker, etc
%     \item NN+Tucker
%     \item via 4-D CP 
%     \item via Tucker
%     \item Resnet et al. don't have FC-layers
% \end{itemize}


There are several methods proposed to compress deep neural networks in these years. \cite{chen2015compressing}  compresses  deep neural networks by employing the hashing trick, because there is redundancy in the weight of DNN \cite{zeiler2014visualizing}. \cite{han2015deep} compresses deep neural networks with pruning, trained quantization and huffman coding, which achieves a high compression ratio in terms of storage.
\cite{hubara2016binarized} proposes the binarized neural networks where the parameters and the activation functions are binarized  in the training process and the gradients are binarized as well. This work can speedup 7 times compared with the traditional CNN.
In addition, there are also some methods aiming to speed up the convolutional layers via low-rank decomposition of the convolutional kernel tensor \cite{lebedev2014speeding,denton2014exploiting,jaderberg2014speeding,kim2015compression}.


Recently, tensor decomposition is getting more and more attention in a wide range of fields, such as signal processing \cite{de2007fourth}, computer vision \cite{shashua2001linear}, numerical analysis \cite{beylkin2002numerical},  and network analysis or recommendation systems \cite{tensorXuYQ15,chen2013exact,LiXWYKL17}. A comprehensive overview about the tensor decomposition can be found in the survey paper \cite{kolda2009tensor}. 
Tensor decomposition has recently been studied in the connection with deep learning, like sharing residual units \cite{yunpeng2017sharing}, speeding up CNNs \cite{lebedev2014speeding}, tensor switching nets \cite{tsai2016tensor}, tensorizing neural networks \cite{novikov2015tensorizing,garipov2016ultimate} and tensor regression networks \cite{kossaifi2017tensor1}.

Concurrent with our work, \cite{kossaifi2017tensor} proposes the TC-layers to substitute the FC-layers, which just perform a transformation along each mode of the input tensors. Therefore, the compression ratio of the parameters is not quite high.
\cite{novikov2015tensorizing} replaces the FC-layers with TT-layers, where the input tensors are reshaped into low-dimensional high-order tensors and the weight matrices are factorized into the corresponding tensor train format.  
Compared with these works, we use the block-term format (BT-format) to replace the weight matrices in the FC-layers, where we can get stronger connections (i.e., higher BT-ranks) with fewer parameters.

It is important to note that there are some neural network architectures without large FC-layers  such as the ResNet \cite{he2016deep}, which aims to designing narrower and deeper networks. The motivation of our proposed model is different from these networks and it is possible to combine the proposed BT-layers with the ResNet. 

%It is important to note that there are some neural network architectures either replacing the FC-layers with 1x1 conv layers, such as the GoogLeNet \cite{szegedy2015going}  or designing narrower and deeper networks, such as the ResNet \cite{he2016deep}. The motivation of our proposed model is different from these networks and perhaps the combination of them  can lead to better performance. 
%researchers try hard to replace the large FC-layers  with 1x1 conv layers 
% \cite{lin2013network} 
%GoogLeNet \cite{szegedy2015going} or  design narrower and deeper architectures, like ResNet \cite{he2016deep}. 
%Our proposed model is motivated differently from these models and perhaps such strategies can be combined together. 
% helps them out this problem as it could remarkably reduce the number of parameters in the FC-layers.


